NavVI: A Telerobotic Simulation with Multimodal Feedback for Visually Impaired Navigation in Warehouse Environments

Industrial warehouses are congested with moving forklifts, shelves and personnel, making robot teleoperation particularly risky and demanding for blind and low-vision (BLV) operators. Although accessible teleoperation plays a key role in inclusive workforce participation, systematic research on its use in industrial environments is limited, and few existing studies barely address multimodal guidance designed for BLV users. We present a novel multimodal guidance simulator that enables BLV users to control a mobile robot through a high-fidelity warehouse environment while simultaneously receiving synchronized visual, auditory, and haptic feedback. The system combines a navigation mesh with regular re-planning so routes remain accurate avoiding collisions as forklifts and human avatars move around the warehouse. Users with low vision are guided with a visible path line towards destination; navigational voice cues with clockwise directions announce upcoming turns, and finally proximity-based haptic feedback notifies the users of static and moving obstacles in the path. This real-time, closed-loop system offers a repeatable testbed and algorithmic reference for accessible teleoperation research. The simulator's design principles can be easily adapted to real robots due to the alignment of its navigation, speech, and haptic modules with commercial hardware, supporting rapid feasibility studies and deployment of inclusive telerobotic tools in actual warehouses.

==> Logging.tex <==
\iffalse
Types of Events Being Monitored
    1. Collision with static obstacles
    2. Collision with dynamic obstacles
    3. Proximity alerts (checking if the robot has entered feedback zones --> radius 5 for haptic, radius 1 for audio feedback triggering)
    4. Goal reached (checking if the robot has collided the stopLayer)

What Information is Logged
    1. Unique user id
    2. Timestamp of the event
    3. No of collision (shelf and obstacles)
    4. Total time to reach the goal from start position 

\fi





% Ayon

\iffalse
During the simulation, when a VI user navigates the robot in the warehouse, they may collide with obstacles. For that reason, we developed a monitoring system which is triggered whenever these events occur. As mentioned previously, we monitor two types of collision events - collision with static obstacles and collision with moving obstacles. We added proximity alerts to the monitoring system in order to check if the robot has entered the feedback zones to avoid these collisions entirely. The feedback zones or colliders refers to the zones that are surrounds the different types obstacles so that if the robot enters in these zones, then the event is triggered. We used radius 5 for haptic feedback triggering and radius 1 for audio feedback triggering. Besides these, the monitoring system is also triggered for the event of reaching the goal, when the robot has reached the destination for the simulation, (ie. by adding a collider to the stopLayer).

All of these events are valuable insights to the feasibility and efficiency of our work. And these insights could be useful for future studies and research. For that reason, we collected these information and stored for future studies. Namely we stored the following information: 1) Unique user ids, 2) Timestamps of these events, 3) No of collisions, 4) Total time to reach the goal from the start position. It is worth mentioning here, for each events we stored the timestamps, user ids and the event type. We strongly believe these data will be useful and help us find the current research gaps of telerobotics operated by VI users.
\fi

%Maisha


